How are attributes expressed in face DCNNs?

As deep networks become increasingly accurate at recognizing faces, it is vital to understand how these networks process faces. While these networks are solely trained to recognize identities, they also contain face related information such as sex, age, and pose of the face. The networks are not trained to learn these attributes. We introduce expressivity as a measure of how much a feature vector informs us about an attribute, where a feature vector can be from internal or final layers of a network. Expressivity is computed by a second neural network whose inputs are features and attributes. The output of the second neural network approximates the mutual information between feature vectors and an attribute. We investigate the expressivity for two different deep convolutional neural network (DCNN) architectures: a Resnet-101 and an Inception Resnet v2. In the final fully connected layer of the networks, we found the order of expressivity for facial attributes to be Age > Sex > Yaw. Additionally, we studied the changes in the encoding of facial attributes over training iterations. We found that as training progresses, expressivities of yaw, sex, and age decrease. Our technique can be a tool for investigating the sources of bias in a network and a step towards explaining the network's identity decisions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> abstract.tex <==
\begin{abstract}
%Deep networks have been widely used for face recognition in the recent past. 
As deep networks become increasingly effective for face recognition, it is now important to understand how these networks  make decisions. Although the direct objective of such networks is recognizing identities, there are several factors that affect the networks' ability to predict identity, such as facial pose, gender, age, etc. We hypothesize that deep networks learn about these attributes during training, even without being explicitly supervised to do so. In this work, we define the expressivity of a given attribute as how easy it is to predict that attribute from a given set of features. We present a technique to approximate the expressivity of identity and three important facial attributes: gender, yaw, and age in a given set of deep features extracted from trained face recognition networks, wherein we estimate the mutual information (MI) between these attributes and feature descriptors. We investigate the presence of attribute-wise expressivity in different layers of a trained network to gain more insight into the hierarchical feed-forward pass of the network. In the final fully connected layer of the networks, we find the following order of expressivity of attributes for which the network does not receive any supervision: Age $>$ Gender $>$ Yaw. Additionally, we also study the emergence of these attributes while the network is being trained to recognize faces. Here, we find that throughout the training process expressivity of facial yaw, age, and gender decreases and that of identity increases. We perform these experiments on two high-performing face recognition network architectures and observe remarkably similar results.%draw some important conclusions.

\end{abstract}

==> abstract_v2.tex <==
\begin{abstract}
%Deep networks have been widely used for face recognition in the recent past. 
As deep networks become increasingly accurate at recognizing faces, it is vital to understand how these networks process faces. While these networks are designed to recognize identities, they also capture face related information such as sex, age, and pose of the face. The networks are not explicitly trained to learn these attributes. We introduce expressivity to measure how much a feature vector informs us about an attribute, where a feature vector can be from internal or final layers of a network. Expressivity is computed from a neural network that approximates the mutual information between a representation and an attribute. We investigate the expressivity of age, sex, and yaw on two different deep convolutional neural network (DCNN) architectures: a Resnet-101 and an Inception Resnet v2.  We report on the expressivity of three attributes on the internal layers of both architectures. In the final fully connected layer of the networks, we found the order of  expressivity for the facial attributes to be Age $>$ Sex $>$ Yaw. Additionally, we studied the changes in the encoding of facial attributes over training iterations. We found that as training progresses, the expressivity of yaw, sex and age decrease. Our experiments demonstrate expressivity as a method for gaining deeper understanding of the workings of DCNNs.

\end{abstract}

==> approach.tex <==
\section{Proposed approach}
\label{sec:approach}
\newcommand{\tabrglayer}{
\begin{tabular}{cc}
% (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
\toprule
Layer & Description\\
\midrule
\texttt{Res4a2b} & 2\textsuperscript{nd} convolutional layer of 7\textsuperscript{th} Res-block \\
\texttt{Res5a2c} & 3\textsuperscript{rd} convolutional layer of 9\textsuperscript{th} Res-block\\
\texttt{Pool5}  & \thead{Final pooling layer which takes in the output of the\\ 11\textsuperscript{th} Res-block \texttt{Res\_5c}}\\
\texttt{FC-L2S} 	& \thead{Final fully connected which takes in the output of \texttt{Pool5} \\and computes $L_2$ softmax activation} \\
%\midrule

\bottomrule
\end{tabular}}
\newcommand{\tabaglayer}{
 \begin{tabular}{cc}
% % (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
 \toprule
 Layer & Description\\
\midrule
\texttt{a9\_concat} & Concatenation layer of 10\textsuperscript{th} inception block \\
\texttt{b5\_concat} & Concatenation layer of 17\textsuperscript{th} inception block \\
\texttt{c3\_concat} & Concatenation layer of 36\textsuperscript{th} inception block \\
\texttt{Pool8x8}  & \thead{Final pooling layer which takes in the output of the\\ convolutional layer after 42\textsuperscript{nd} inception block \texttt{c10}}\\
\texttt{FC-L2S} 	& \thead{Final fully connected which takes in the output of\\ \texttt{Pool8x8} and computes $L_2$ softmax activation}\\
%\midrule
 \bottomrule
 \end{tabular}}
\begin{table}%
  \centering
  \subfloat[][Network A]{\tabrglayer}%
  \qquad
  \subfloat[][Network B]{\tabaglayer}
  \caption{Brief descriptions of the layers used to compute expressivity in both the networks. More architectural details are provided in \cite{ranjan2019fast}.}
  \label{tab:des_layers}
  %\vspace{-0.8cm}
\end{table}
\begin{figure}
{\centering
\subfloat[]{\includegraphics[width = 0.5\linewidth, height = 40mm]{images/yawdis_v2.png}}
\subfloat[]{\includegraphics[width = 0.5\linewidth, height = 40mm]{images/agedis_v2.png}}
\caption{\small IJB-C dataset \cite{maze2018iarpa} shows enough variation with respect to (a.) Yaw, (b.) Age, which is required to compute expressivity of age and yaw, in a given set of IJB-C features.}
\label{fig:dis}
%\vspace{-0.5cm}
}
\end{figure} 
 \begin{figure}
 \centering
    %\includegraphics[width=0.5\linewidth, height=5cm] {images/template_net.pdf}
    \includegraphics[width=2in] {images/template_net.pdf}
    \caption{\small We use a consistent network architecture to compute expressivity of $m-$dimensional features $F$, augmented with an attribute vector $A$. More details in Sec. \ref{subsec:proto} }
    \label{fig:template}
    \vspace{-0.55cm}
\end{figure}
\subsection{Networks and datasets used}
To compute the expressivity of identity or attribute $A$ in a given set of features $F$, we extract the features $F$ using the following networks :\\
(1) \textbf{Network A} (Resnet-101 architecture) : The architecture is described in \cite{ranjan2019fast}. For investigating hierarchical course of the feedforward pass, we use a version of this network trained on a combined dataset of all the MS-Celeb-1M and UMD Faces images. For this trained network, we compute expressivity of attributes using features from these layers : \verb|Res4a2b, Res5a2c, Pool5, FC-L2S|.\\
(2) \textbf{Network B} (Inception Resnet v2 architecture).  The architecture is described in \cite{ranjan2019fast}. The training dataset of this network is same as that of Network A. We explore the following layers in the network: \verb|a9_concat, b5_concat, c3_concat, Pool8x8|, \verb|FC-L2S|.\\
Layer-wise details for both the networks are provided in Table \ref{tab:des_layers}.
For computing expressivity, we use IJB-C \cite{maze2018iarpa} as our test dataset. IJB-C dataset consists of 3531 identities with a total of 31,334 still images and 117,542 video frames collected in unconstrained settings. We extract the IJB-C features $F$ from different layers of aforementioned trained networks.  For computing the corresponding attributes $A$, we use the All-in-one network \cite{ranjan2017all}. 
\subsection{Attributes used}
 We compute the expressivity of identity and three attributes : yaw, sex, age in the extracted IJB-C features. To compute the yaw, sex and age of the corresponding IJB-C images, we use the All-in-one deep CNN proposed in \cite{ranjan2017all}, which simultaneously performs face detection, landmarks localization, pose estimation, sex recognition, smile detection, age estimation and face identification and verification. In Figure \ref{fig:dis}, we verify that the IJB-C datasets show enough variation with respect to yaw and age, so that we can insure that expressivity (which is a lower bound estimate of mutual information) is an accurate indicator of the predictability of the corresponding attributes. The IJB-C dataset consists of 2203 male and 1328 female identities, which ensures that sufficient sex variation exists. 
 
 We now briefly explain the attribute vector $A$ introduced in Section \ref{sec:expressivity}. When considering sex, the vector $A$ consists of probability values of the sex being male (\verb|PR_MALE|), which are the outputs of All-in-One network in \cite{ranjan2017all}. When considering identity, $A$ is a discrete vector, where each element is a numerical identity label. We generate the attribute vector $A$ for yaw (in degrees) and age (in years) in a similar manner. The exact methodology to compute the expressivity using the feature descriptors and their respective attribute vector is provided in the next subsection.
\begin{algorithm}[H]
\floatname{algorithm}{Protocol}
\caption{Computing expressivity using flattened features}
\label{protocol1}
\begin{algorithmic}[1]
\STATE \textbf{Input}: layer $L$,  
\STATE \textbf{Input}: Set of $n$ images $I$
\STATE \textbf{Input}: attribute vector $A\in \mathbb{R}^{n \times 1}$
\STATE \textbf{Initialize} $E = []$
\STATE For a given image $i \in I$, extract feature $f_i$
\STATE Augmentation step $X = [F | A]$, where $F=[f_1,f_2 \ldots f_n]^T$
\FOR {$iter:$ 1 to M}
%\bindent
\STATE Initialize MINE network according to dimensions of $X$
\STATE $E\leftarrow$MINE($X$)
%\eindent
\ENDFOR
\STATE \textbf{return} Expressivity = Average($E$)
\end{algorithmic}
\end{algorithm} 
\begin{algorithm}[H]
\floatname{algorithm}{Protocol}
\caption{Computing expressivity using unflattened feature maps}
\label{protocol2}
\begin{algorithmic}[1]
\STATE \textbf{Input}: layer $L$, with $k$ channels, each of dimension $d\times d$
\STATE \textbf{Input}: Set of $n$ images $I$
\STATE \textbf{Input}: attribute vector $A\in \mathbb{R}^{n \times 1}$
\STATE \textbf{Initialize} $E = []$
\STATE $S=$ Subset of randomly selected $z$ (out of $k$) channels 
\STATE For a given image $i$, vectorize and concatenate all $z$ maps in $S$, to generate vector $f_i$ of dimension $m\times1$, where $m=d*d*z$
\STATE Augmentation step $X = [F | A]$ where $F=[f_1,f_2 \ldots f_n]^T$
\FOR {$iter:$ 1 to M}
%\bindent
\STATE Initialize MINE with input dimensions of $X \in \mathbb{R}^{n\times m+1}$
\STATE $E\leftarrow$MINE($X$)
%\eindent
\ENDFOR
\STATE \textbf{return} Expressivity = Average($E$)
\end{algorithmic}
\end{algorithm}
\subsection{Protocols to compute expressivity}
\label{subsec:proto}
\vspace{-0.25cm}
In this work, we define expressivity as a lower bound approximation of MINE, as explained in section \ref{sec:expressivity}. We consider two protocols (described above): Protocol-1, to compute the expressivity of attributes in flattened features (i.e. features from fully connected or pooling layers which are extracted as vectors). Protocol-2, to compute the expressivity of attributes in unflattened feature maps (i.e. feature maps from a convolutional layer which are extracted as 2D channels). For both of these protocols, we need a set of $n$ images, and their corresponding attributes $A\in \mathbb{R}^{n\times 1}$. In step 8 of Protocol-1 and step 9 of Protocol-2, we initialize a MINE approximation network according to the input dimension of the augmented matrix. As explained in Section \ref{sec:expressivity}, we train the network to compute the lower bound approximation of mutual information between features $F$ and attribute $A$. We use a simple multi layer perceptron (MLP) network, described in Figure \ref{fig:template}, for computing $T_\theta$ in (\ref{eq:loss}). The network consists of two hidden layers with 256 and 128 units. These layers are followed by ELU activations. We use this architecture consistent throughout our experiments. When using different sets of features for $F$, the only architectural changes in the network are made in the input layer dimension, according to the feature dimension. The network is trained until the loss in (\ref{eq:loss}) converges and expressivity is computed using the protocols. In step 8 in Protocol-1 and step 9 in Protocol-2 we initialize and train the MINE network multiple times ($M$) to increase number parameter sets $\theta$ in (\ref{eq:mi}), among which the supremum is to be found. In all our experiments, we use $M=16$. Also, in step 5 of Protocol-2 we select only a subset of features maps (channels), as mentioned in \cite{alain2016understanding}. Note that, for any attribute vector $A$ (yaw/identity/age/sex), we use the same feature subset $S$.

Apart from analyzing the network layer features, we also investigate the presence of various attributes in the raw RGB face image in Section \ref{sec:experiments}. For this, we average the R,G and B channels to generate a grayscale image. Following this, we vectorize the image and use it as feature $f_i$ in Protocol-1.
\subsection{Training linear classifiers}
To verify that expressivity correctly indicates the ease of predictability of attributes in features, we show its correlation with accuracy/error-rates of linear classifiers trained on the corresponding features. We randomly select a subset of 5000 IJB-C images and extract their features. To train the linear classifier we use 3000 features and test it on 2000 features. This is a trivial task for flattened features. However, to compute the accuracy/error rate in feature maps from higher layers of the network, we use the same subset $S$ of feature maps as selected in step 5 of Protocol-2. Following this, we vectorize and concatenate them as in Step 7. We provide more specific details in the next section.

==> experiments.tex <==

\section{Experiments}
\label{sec:experiments}
\newcommand{\tabrg}{
\begin{tabular}{ccccc}
% (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
\toprule
Layer & Dim. ($c\times d\times d$)& Protocol & $z$ & Feat. dim\\
\midrule
\texttt{Res4a2b} &$1024\times14\times14$&2&11&2156\\
\texttt{Res5a2c}  &$2048\times7\times7$&2&42&2057\\
\texttt{Pool5}  &2048	&1&-&2048\\
\texttt{FC-L2S} 	&512	&1&-&512\\
%\midrule

\bottomrule
\end{tabular}}
\newcommand{\tabag}{
 \begin{tabular}{ccccc}
% % (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
 \toprule
 Layer & Dim. ($c\times d\times d$)& Protocol & $z$ & Feat. dim\\
 \midrule
 \texttt{a9\_concat}&$128\times35\times35$&2&3&3675\\
 \texttt{b5\_concat}  &$384\times17\times17$&2&13&3757\\
 \texttt{c3\_concat}  &$128\times8\times8$&2&59&3776\\
 \texttt{Pool8x8}  &1536	&1&-&1536\\
 \texttt{FC-L2S}	&512	&1&-&512\\
 \bottomrule
 \end{tabular}}
 
\begin{table}%
  \centering
  \subfloat[][Network A]{\tabrg}%
  \qquad
  \subfloat[][Network B]{\tabag}
  \caption{\small Network A and B layers used to compute expressivity. $c$ : number of channels in a given layer, $d$: channel dimension, $z$ : Number of channels selected out of $c$ channels, to generate a subset of features}%
  \label{tab:layers}%
\end{table}
%Network A and B layers used to compute expressivity. $c$ : number of channels in a given layer, $d$: channel dimension, $z$ : Number of channels selected out of $c$ channels, to generate a subset of features
Using the protocols described in Section \ref{sec:approach} and the expressivity measure defined in \ref{sec:expressivity}, we extract features from different layers of Networks A and B and use them to train a network (Figure \ref{fig:template}) to compute expressivity of various attributes.
\subsection{Hierarchical course of feedforward pass}
\label{subsec:hierar}
 Table \ref{tab:layers} shows the network layers explored, along with the final dimension of the features used for computing expressivity for both the networks. The layerwise expressivity values for Networks A and B are shown in Figure \ref{fig:hierar}. It should be noted that both the networks were trained using identity-supervision and no supervision based on pose, sex and age. Our inference is listed as follows:
\begin{itemize}[leftmargin=*]
    \item In both networks A and B, we find that the expressivity of yaw, sex and age is high and that of identity is the lowest in the shallower layers (\verb|Res4a2b, Res5a2c| in Network A; \verb|a9_concat, b5_concat, c3_concat| in Network B) and input image. This shows that yaw and sex are high level face features as compared to identity, which cannot be extracted using shallow layers.
    \item As we examine the deepest layer (FC-L2S), the expressivity of yaw and sex attain their lowest values, whereas identity and age have very high expressivity. This shows that identity and age are more fine grained features compared to other attributes.
    \item There is a rapid increase in the identity expressivity from the pooling to fully connected layers, in both the networks.
    \item Comparing the expressivity values of all attributes except identity in the final layer, we can infer that for identity recognition, yaw is the least important and age is the most important attribute.
\end{itemize}

There are three reasons for the relatively high expressivity of the
age when compared to the other attributes. 

First, in the IJB-C dataset most of the images were acquired over a short
period of time, therefore, it can happen that a given age is predictive of an identity. Second, we used an automated algorithm \cite{ranjan2017all} to estimate the age, and therefore it is computed from the appearance of the face. All attributes were computed automatically, but we can expect that in relative terms the age is the least accurate of all attributes automatically computed. Third, the entropy of the age (Fig. \ref{fig:dis}(b)) is higher than the entropy of the other attributes and this could increase the mutual information component
of the expressivity.

\textbf{Discussion of the data processing inequality}: The data processing inequality (DPI) \cite{cover2012elements} states that for three random variables $P, Q, R$ forming a Markov chain $P\longrightarrow Q\longrightarrow R$, $$\text{MI}(P,Q)\geq \text{MI}(P,R). $$

The data processing inequality formalizes the concept that no processing of data can increase mutual information. To make this more concrete, let $P$ be any random variable (e.g. sex, yaw, identity), and let $Q,R$ be features for different layers in a network where $R$ is a deterministic function of $Q$, i.e. $R$ is deeper than $Q$. Since $R$ is a function of $Q$ then $P,Q,R$ forms a Markov chain \cite{cover2012elements}. It follows from the DPI that the information about $P$ contained in the features cannot increase as we go deeper. %For networks with random noise between features, like a variational autoencoder, as long as $R$ given $Q$ is independent of $P$ then $P,Q,R$ forms a Markov chain and the DPI still applies.

% We consider an input to a network to be the result of a random process which is defined by a world state random variable. Such a world state includes everything necessary to produce an image, as well as everything one could hope to measure about the image (e.g. sex, yaw, identity). Denote this world state as $P$. Let $Q$ be either the input image or the activation map of a layer in the network and let $R$ be the activation map of a deeper layer in the network. By deeper, we mean specifically that $R$ is a deterministic function of $Q$. Since $R$ is a function of $Q$ it follows that $P, Q, R$ forms a Markov chain \cite{cover2012elements}.

The expressivity results in Figure \ref{fig:hierar} are not monotonically decreasing, which might seem like a contradiction to DPI. However, as pointed out in \cite{alain2016understanding}, the features in our context denote \textit{representation}, rather than \textit{information content} described in Information Theory. \textit{Representations} are more closely related to predictability of a specific attribute, as compared to information-theoretic content. Hence, in this work, expressivity refers to the predictability of a certain attribute, rather than its theoretical information content.

% Here we consider $P$ to be the original image data, which contains maximum information with respect to any attribute. Let $Q, R$ be features from two different layers of the network such that layer corresponding to $R$ is deeper than that of $Q$. According to this, for any attribute, the mutual information of features of any layer should be less than that of its parent layer.  This contradicts the results shown in Figure \ref{fig:hierar}.  However, as pointed out in \cite{alain2016understanding}, the features in our context denote \textit{representation}, rather than \textit{information content} described in Information Theory. \textit{Representations} are more closely related to predictability of a specific attribute, as compared to information-theoretic content. Hence, in this work, information is used to refer predictability of a certain attribute, as mentioned in Section \ref{sec:intro}. \\

\begin{table}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}
% (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
\toprule
Layer & \thead{Sex \\classfic\textsuperscript{n} acc.} & \thead{Sex \\expressivity} & \thead{Yaw \\regress\textsuperscript{n} error} & \thead{Yaw \\expressivity}\\
\midrule
\texttt{Res4a2b} &0.937&1.12&11.42&1.36\\
\texttt{Res5a2c}  &\textcolor{green}{0.951}&\textcolor{green}{1.26}&\textcolor{green}{8.64}&\textcolor{green}{1.48}\\
\texttt{Pool5}  & 0.938 &1.17&11.57&1.23 \\
\texttt{FC-L2S} 	&\textcolor{red}{0.803}&\textcolor{red}{0.89}&\textcolor{red}{11.65}&\textcolor{red}{0.59}\\
\bottomrule
\end{tabular}
}
%\vspace{.5em}
\caption{\small Comparison of sex classification accuracy and yaw regression error with their corresponding expressivity values, in different layers of Network A. The highest accuracy (or lowest error) corresponds to highest expressivity and lowest accuracy (or highest error) corresponds to lowest expressivity.}
\label{table:rg1_compare}
% \vspace{-0.8cm}
\end{table}
\textbf{Relation with linear separability}: Alain and Bengio \cite{alain2016understanding} show that the linear separability of features with respect to output classes, which provided supervision, monotonically increases as we go deeper into the network. From Figure \ref{fig:hierar}, we find this to be true for expressivity identity as well, which provided supervision during training . \\

In order to ensure that the expressivity values correlate with predictability, we compute the accuracy/error rate obtained by training a linear classifier and testing it directly using features from the aforementioned layers in Network A, as explained Section \ref{sec:approach}. To analyze the sex expressivity values, we first train a simple logistic regression model on 3000 randomly selected features (extracted from IJB-C images) and evaluate its classification accuracy on 2000 IJB-C features. Similarly, for analyzing yaw expressivity values, we train a linear regression on the randomly selected training features and evaluate the regression error on test features. The corresponding results are presented in Table \ref{table:rg1_compare}, from which we can infer that expressivity values do correlate with classification accuracy of sex and regression error of yaw.
\begin{figure*}
   \centering
   \subfloat[][Network %A]{\includegraphics[width=0.45\linewidth]{images/rg1_dissect.png}}
   A]{\includegraphics[width=3in]{images/rg1_layer_new.png}}
   \rulesep
    \subfloat[][Network %B]{\includegraphics[width=0.40\linewidth]{images/ag1_dissect.png}}
    B]{\includegraphics[width=2.85in]{images/ag1_layer_new.png}}
    \caption{\small Expressivity of identity, age, sex and yaw in input image and layerwise features from both the networks. The source image for face in this figure is attributed to Eva Rinaldi under the
\href{https://creativecommons.org/licenses/by-sa/2.0/deed.en}{[cc-by-sa-2.0]} creative commons licenses respectively. The face was cropped from the source image.}
    \label{fig:hierar}
    %URL for image is https://commons.wikimedia.org/wiki/File:Sandra_Bullock_(9192364254).jpg
\end{figure*}
\vspace{-0.2cm}
\subsection{Temporal course of training}
\begin{figure*}
    \centering
    \subfloat[]{\includegraphics[width=0.515\linewidth]{images/temporal_rg1.png}}
    \subfloat[]{\includegraphics[width=0.495\linewidth]{images/temporal_ag1.png}}
    \caption{\small Expressivity of identity, age, sex and yaw in final layer (FC-L2S) features of a.) Network A and b.) Network B.  Decreasing expressivity of task irrelevant attributes (yaw, age, sex) is a part of training. Observed rate of decrease : Age $<$ Sex $<$ Yaw }
    \label{fig:temporal}
\end{figure*}
We also analyze the training process of Network A and B and investigate the changes in the expressivity of yaw, sex, identity and age in the final layer (FC-L2S) of these networks with respect to its training iterations. The features at all iterations ($>0$) are 512 dimensional and are flattened and Protocol-1 is used for computing attribute-wise expressivity, along with specifications for FC-L2S mentioned in Table \ref{tab:layers}. The features at iteration 0, represent the final layer features of the networks trained on ImageNet \cite{Imagenet}, without the final fully connected layer for identity recognition. These features are therefore 2048 and 1536 dimensional for networks A and B respectively. The results are presented in Figure \ref{fig:temporal}.  Our observations are listed below:
\begin{itemize}[leftmargin=*]
    \item We find that the expressivity of yaw, age and sex reach their peak values in the first $~$25000 iterations for Network A and $~$40000 iterations for Network B, to learn the general concept of facial pose, age and sex.
    \item Following that, we find that the yaw expressivity decreases rapidly as the training proceeds, showing that making features almost agnostic to pose variance is an essential part of the training process. %the network attempts to abstract away the pose variance.
    \item For both networks A and B, the expressivity of age and sex decreases slightly after their corresponding expressivity peaks are attained, during the course of training. However, compared to yaw, the rate of decay in the expressivity of age and sex is low. This shows that age and sex are more important for identity recognition than face yaw.
    \item Observing the expressivity values in the final iteration, we can infer that for identity recognition, the following is the order of relevance of attributes for which the network does not receive any supervision : Age $>$ Sex $>$ Yaw. The opposite of this order is observed in the rate by which the expressivity values of yaw, age and sex decreases, i.e. the rate of decrease is : Age $<$ Sex $<$ Yaw. This is true for both networks A and B.
    \item The expressivity of identity generally increases during training for both networks A and B.
    \item Features extracted from the final layer of Iteration 0 model (Imagenet features), express identity better than other attributes. This is because the Imagenet features express `objectness', which is closely related to identity as compared to other attributes (yaw, age, sex).  
\end{itemize}
Similar to what we did in Section \ref{subsec:hierar}, we compare the expressivity values to the corresponding accuracy/error rates by training and testing linear classifiers directly on the final fully connected layer features. The results are presented in Table \ref{table:rg1_temporal_compare}, where we again find that there exists correlation between expressivity values and sex classification accuracy and age/yaw regression error. 
\begin{table}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc|cc}
% (10,99.2)(20,99.55)(30,99.18)(40,98.72)(50,98.10)(60,97.22)(70,95.49)(80,92.86)(90,90.18)(100,87.75)
\toprule
Iteration & \thead{Sex \\acc.} & \thead{Sex \\expr.} & \thead{Yaw \\ error} & \thead{Yaw \\expr.}&\thead{Age \\ error} & \thead{Age \\expr.}\\
\midrule
$T_1$ &\textcolor{green}{0.90}&\textcolor{green}{1.03}&\textcolor{green}{9.40}&\textcolor{green}{1.13}&8.06&1.22\\
$T_2$  &0.82&1.01&11.27&0.68&\textcolor{green}{7.70}&\textcolor{green}{1.39}\\
$T_3$  & \textcolor{red}{0.80}&\textcolor{red}{0.89}&\textcolor{red}{11.65}&\textcolor{red}{0.59}&\textcolor{red}{8.11}&\textcolor{red}{1.19}\\
\bottomrule
\end{tabular}
}
\caption{\small Comparison of sex classification accuracy and age/yaw regression error with their corresponding expressivity values in 3 iterations $T_1,T_2,T_3$. For yaw, $T_1,T_2,T_3=25k,100k,200k$ iterations. For sex, $25k,125k,200k$. For age $50k,100k,200k$}
%\vspace{-1cm}
\label{table:rg1_temporal_compare}
\end{table}
\subsection{Advantage of expressivity over other techniques}
% if the question is, what kind of information does a network learn interms of any given attribute
%comparative study, any concept (discrete / physical)
%good for : how much info does network learn about a given concept discrete / continuous
%not good for : knowing if a certain class is affected by a given concept
% 
The following are the advantages of Expressivity over existing interpretability techniques:\\
\textbf{Comparison of several attributes}: Comparing expressivity of different attributes in a given set of features is important for understanding the information organization in a trained network. As shown in Figures \ref{fig:temporal} and \ref{fig:hierar}, expressivity helps put the predictability of various attributes on the sample scale, thus enabling their comparisons. This cannot be achieved by directly using the accuracy/error rates of linear classifiers, as different attributes have different scales and evaluation metrics. \\
\textbf{Useful for any physical concept (discrete/continuous)}: Although we used expressivity to analyze face recognition networks in terms of facial attributes, it can be used for a network with respect to any physical attribute. For instance, we can compute the expressivity of `stripes' concept in a set of features $F$ if we have a binary attribute vector $A$, denoting the presence or absence of `stripes'. This is similar to TCAVs \cite{kim2017interpretability}. However, TCAVs cannot be directly used to quantify the content of continuous concept (like pose angle), since we need images with which demonstrate absence of that concept to train CAVs, and this is not trivial for concepts like pose angle, age etc.  \\
\textbf{No dependence on training classes}:  Methods like \cite{kim2017interpretability} and \cite{selvaraju2017grad} require computing change of logit values. However, for images not in training classes, this value is not meaningful. While using expressivity to quantify the predictability of an attribute in a given set of features, we do not require features to correspond to any training class(es).  \\
\vspace{-0.5cm}
\subsection{Relation with information bottleneck theory}
Saxe \emph{et al.} \cite{saxe2018information} provide a response to the Information Bottleneck theory \cite{shwartz2017opening}, and claim that when an input domain consists of a subset of task-relevant and task-irrelevant information, hidden representations do compress the task-irrelevant information. In our context, identity is the task-relevant information, since the networks only receive identity supervision. The task-irrelevant information includes are yaw, age and sex information. In our work, we concur with the claims of \cite{saxe2018information}. It can be seen in Figures \ref{fig:temporal} the expressivity of task-irrelevant attributes (yaw, age, sex) in the final layer decreases as we train the network, depicting the `compression' phase. This occurs while the identity expressivity increases as the training progresses, which corresponds to the `fitting' phase of the network. Hence, we also verify another result in \cite{saxe2018information}, that this compression happens concurrently with the fitting process rather than during a subsequent compression period.

==> expressivity.tex <==
\section{Expressivity}
\label{sec:expressivity}
Predictability of facial attributes/identities in a given set of face descriptors indicates the attribute-relevant information content encoded in the descriptors. To estimate this information content, we intend to use Mutual Information (MI). MI between two random variables is a measure of the amount of information that can be obtained for one random variable by observing the other variable. Therefore, if we estimate MI between face descriptors and their corresponding identities/attributes, we can estimate the information content (and hence the predictability) of these identities/attributes in the given descriptors. Since MI can be computed for both categorical and continuous attributes, an estimate based on MI  provides a  measure which is consistent across categorical and continuous attributes. 

MI between two random variables ($V_1, V_2$) is given as:
\begin{equation}
    I(V_1,V_2) = D_{KL}(\mathbb{P}_{V_1,V_2}\|\mathbb{P}_{V_1} \otimes \mathbb{P}_{V_2})
\end{equation}
where, $D_{KL}$ represents the Kullback-Leibler divergence, $\mathbb{P}_{V_1,V_2}$ denotes the joint probability distribution, $\mathbb{P}_{V_1}$ and $\mathbb{P}_{V_2}$ denote the marginal distributions, and $\mathbb{P}_{V_1} \otimes \mathbb{P}_{V_2}$ represents the product of the marginal distributions. Tishby and Zaslavsky \cite{tishby2015deep} show that each layer in a deep network can be quantified by the amount of mutual information (MI) it retains on the input variable, on the (desired) output variable, as well as on the predicted output of the network. However, as mentioned in \cite{belghazi2018mine}, computing MI is not a trivial task. Most of the existing non-parametric approaches for estimating MI do not scale with the dimensionality of variables. Belghazi \emph{et al.} \cite{belghazi2018mine} propose MINE to estimate MI between high dimensional continuous variables using gradient descent over neural networks.
The neural information measure has been defined in \cite{belghazi2018mine} as follows.
\begin{equation}
    I_\Theta(F, A) = \underset{\theta \in \Theta}{\text{sup}} ~\mathbb{E}_{\mathbb{P}_{FA}}[T_\theta] - \text{log}(\mathbb{E}_{\mathbb{P}_{F}\otimes \mathbb{P_A}}[e^{T_\theta}])
\label{eq:mi}
\end{equation}
where $F, A$ are the variables whose mutual information is to be estimated, $\theta \in \Theta$ represents parameters in a network computing a function $T_\theta : F,A \longrightarrow \mathbb{R}$. As proved in \cite{belghazi2018mine}, the MINE estimate provides a lower bound estimate to the actual MI. 

In the context of our work, we define `Expressivity' of $A$ in $F$ as the aforementioned information measure (Equation \ref{eq:mi}). We use MINE to compute the expressivity of face identity and various facial attributes $A$ (discrete and continuous) in a given set of face descriptors $F$. Although face identity is not strictly a face `attribute', we treat it in the same way as a face attribute. Therefore, in this work, attribute $A$ collectively refers to identity and facial attributes like pose, sex etc.\\

Following the protocols detailed in \cite{belghazi2018mine}, we briefly explain how gradient descent over a neural network can be used to compute expressivity. Let $f_i \in \mathbb{R}^m$ denote $i^{th}$ feature in a batch $B$ of size $b$ (i.e. $|B| = b$), and $a_i \in \mathbb{R}$ denote the corresponding attribute value. The set $\{(f_i, a_i)\}^{b}_{i=1}$ represents the $b$ elements sampled from the joint distribution ($f_i, a_i \sim \mathbb{P}_{FA}$). Similarly ${\{\Tilde{a_i}\}^{b}_{i=1}}$ represents $b$ attribute values sampled from a marginal distribution ($\Tilde{a_i} \sim \mathbb{P}_{A}$).  To estimate the the neural information in \ref{eq:mi}, we compute the expectation over joint and marginal distribution as follows :
$$\mathbb{E}_{\mathbb{P}^{(b)}_{FA}}[T_\theta] =\frac{1}{b}\sum ^{b}_{i=1} T_{\theta}(f_i, a_i) $$
$$\mathbb{E}_{\mathbb{P}^{(b)}_{F}\otimes \mathbb{P}^{(b)}_A}[e^{T_\theta}] =\frac{1}{b}\sum ^{b}_{i=1} e^{T_{\theta}(f_i, \Tilde{a}_i)} $$

where $b$ is the number of features in a batch $B$ whose mutual information to be computed with their corresponding attributes. We use a network with parameter set $\theta$ (see Fig. \ref{fig:template}) to compute the aforementioned arbitrary function $T_{\theta}(f_i, a_i)$ and $T_{\theta}(f_i, \Tilde{a}_i)$. By substituting $\mathbb{E}_{\mathbb{P}_{FA}}[T_\theta]$ and $\mathbb{E}_{\mathbb{P}_{F}\otimes \mathbb{P}_A}[e^{T_\theta}]$ in Eq. \ref{eq:mi} , the function $\mathcal{V}(\theta)$ is computed as:
\begin{equation}
     \mathcal{V}(\theta) = \frac{1}{b}\sum ^{b}_{i=1} T_{\theta}(f_i, a_i) - \text{log}(\frac{1}{b}\sum ^{b}_{i=1} e^{T_{\theta}(f_i, \Tilde{a}_i)})
\label{eq:nu}
\end{equation}
 As mentioned in \cite{belghazi2018mine}, the supremum of $\mathcal{V}(\theta)$ with respect to parameter set $\theta$ is a lower bound approximation of the mutual information between features $F$ and attributes $A$. Hence we use the following function $L$  as our objective function to train the network $N$.
\begin{equation}
    L(\theta)=-\mathcal{V}(\theta)
\label{eq:loss}
\end{equation}
\begin{equation}
    \nabla_\theta L(\theta) = - \Bigg( \mathbb{E}_{\mathbb{P}^{(b)}_{FA}} [\nabla T_\theta] - \frac{\mathbb{E}_{\mathbb{P}^{(b)}_{F} \otimes \mathbb{P}^{(b)}_{A}}[\nabla T_\theta e^{T_{\theta}}]}{\mathbb{E}_{\mathbb{P}^{(b)}_{F} \otimes \mathbb{P}^{(b)}_{A}}[e^{T_\theta}]}\Bigg)
\label{eq:grad}
\end{equation}
 At every training iteration, we use a different parameter set $\theta$ to compute the function $T_{\theta}$. As the training proceeds, the network minimizes (\ref{eq:loss}), thus maximizing $\mathcal{V}(\theta)$ with respect to $\theta$. This is equivalent to computing the supremum of $\mathcal{V}(\theta)$. Hence, the final value of $\mathcal{V}(\theta)$ at convergence is an approximation of Expressivity. (Eq. \ref{eq:mi})
 
 
 In equations (\ref{eq:nu}) and (\ref{eq:loss}), the objective function (and the lower bound of mutual information) is computed in a batch and not on the given set of features and their attribute values, thus making the gradients biased towards the minibatch, rather than the full batch. This issue has been identified in \cite{belghazi2018mine}, and can be mitigated by replacing the expectation term in the denominator of gradient update (\ref{eq:grad}) by an exponential moving average. More theoretical details related to this approximation of mutual information is provided in \cite{belghazi2018mine}.


==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Significant research has been done in training state-of-the-art face recognition networks  in the past few years \cite{schroff2015facenet,taigman2014deepface,ranjan2019fast,deng2018arcface,bansal2018deep}. As such networks find more usage in the real world, the requirement for the networks to be more explainable and interpretable becomes more pressing.  %In order to make the predictions of face recognition more acceptable, it is important to gain insights into how it makes decisions. 
We believe that this can be done by investigating how expressive the network features are with respect to important facial attributes. Conceptually, \textit{expressivity} of an entity can be defined as the ease with which that entity can be predicted using a given set of features. We provide a more precise definition in Section \ref{sec:expressivity}.


In this paper we pose the following questions: Which layers in a trained face recognition network encode the maximum facial pose expressivity? Which layer encapsulates the maximum identity expressivity? How much information about gender and age does the network learn during training? To answer such questions, we need a tool to quantify the information content of any attribute in a given set of network features. We present such a tool, and demonstrate its usage in analyzing the expressivity encoded in existing face recognition networks.  Investigating various layers of a network and its training process can help to insure that the network does not pick up any untoward bias or make decisions based on the expressivity of any protected attributes. Also, using layer wise expressivity, we can determine which layer to use for predicting a specific attribute.
\begin{figure}
    \includegraphics[width=\linewidth] {images/fg_teaser.pdf}
    \caption{We propose to `explain' a trained face recognition network by computing expressivity of various facial attributes in a given set of face descriptors}
    \label{fig:teaser}
\end{figure}

A simple technique to compute expressivity of a face  attribute in a given set of features is to train a classifier on these features to predict the aforementioned attributes, and use the accuracy/error rate as an indicator of its predictability. However,  this is not a good approximation because: (i.) The scale of error/accuracy varies with the attribute under consideration. For example: Gender predictability approximation requires computation of classification performance, whereas yaw predictability requires measurement of regression performance, which is why the expressivity of gender and yaw cannot be compared simultaneously. (ii.) The error/accuracy depends on the model/classifier being used, and thus does not solely capture the predictability of attributes in a given set of features. 

Hence, we require a more principled technique to approximate the expressivity of various attributes which makes face recognition network interpretable. %Although interpretability of face recognition networks has not been exclusively researched before, there exist several works which analyze interpretability of a network with respect to various concepts. For instance, \cite{kim2017interpretability} proposes a method to approximate the sensitivity of network activation in terms of existence of single physical concepts like stripes, neck tie etc. However, information content of concepts which exist universally and have continuous values (such as angular orientation)  cannot be directly estimated using this approach.
An ideal tool for probing should be uniform across different attributes, whose information we aim to approximate. In this work, we propose to interpret a network by quantifying the expressivity of various attributes vector as a function of the network's features, using a lower bound approximation of their mutual information (MI), (see Figure \ref{fig:teaser}). We believe that if the given features are appropriately sampled, their expressivity of various attributes should be a good indicator of their predictability. %Using this method, we intend to probe various layers of a network and monitor its training process. Here, we do not propose a method to train face recognition network which preserves explainability. Rather, we present a technique to examine trained networks and their historical snapshots.

We make the following contributions in this paper: 
\begin{enumerate}[leftmargin=*]
    \item We define `expressivity' of an entity as a measure of its predictability, and propose an approach to estimate the expressivity of yaw, age, gender and identity, in a given set of face descriptors.
    \item We analyse expressivity of several attributes in various layers of commonly used face recognition networks. The following order of expressivity holds for attributes for which the network does not receive supervision : Age $>$ Gender $>$ Yaw, in the final fully connected layer.
    \item We also monitor the changes in the expressivity of attributes in the final fully connected layer of a network as its training progresses. We find that during training, the expressivity of yaw, gender and age decreases (un-learned), while that of identity increases. The rate of un-learning is Age $<$ Gender $<$ Yaw.
\end{enumerate}
%(1) We define `expressivity' of an entity as a measure of its predictability, and propose an approach to estimate the expressivity of yaw, age, gender and identity, in a given set of face descriptors. This approach is uniform across all attributes being examined, discrete or continuous. (2) Using the aforementioned approach, we study the predictability of several attributes in various layers of commonly used face recognition networks. We find that the following order of expressivity holds for attributes for which the network does not receive supervision : Age $>$ Gender $>$ Yaw. (3) We also monitor the changes in the expressivity of attributes in the final fully connected layer of a network as its training progresses. We observe that the network generally increases identity expressivity in the final layer. We also find that the network first learns yaw, age and gender information, and then un-learns this for the remaining iterations. However, it un-learns yaw information more rapidly than gender and age.


==> intro_v2.tex <==
\newcommand{\tcr}[1]{\textcolor{red}{#1}}
\newcommand{\pjp}[1]{\textcolor{red}{#1}}
\newcommand{\prithvi}[1]{\textcolor{blue}{#1}}

\section{Introduction}
\label{sec:intro}

From a quick glance of a face image, the viewer can discern the gender, age, race of the person, the pose and lighting of the face, and maybe the details of the location where the photo was taken.   
Deep convolutional neural networks (DCNN)-based face algorithms generate a representation that encodes the identity of face.
Along with identity, the representation encodes additional information including gender, pose, age, illumination direction \cite{hill2018deep,DBLP:journals/corr/abs-1904-01219,parde2017face}.  For trained networks, how much information about  facial attributes are captured in the internal layers of the network?  How does the encoding of facial attributes evolve during training?  We address both these questions.


Understanding how face attributes are expressed in different layers of a DCNN and how they evolve during training has both scientific and societal importance. 
Since DCNN-based face recognition systems are fielded in the real-world, the need for these networks to be explainable is pressing.  Understanding how all layers encode attributes serves as a basis for explaining identification decisions.
 The ability to  discern important attributes from the final layer is not the final word; it may be possible to discern them from the interior of a network.  For example, the face representation maybe gender or race neutral; however, this information could be encoded in the internal layers of the network.  From a scientific perspective, knowing the relative importance of attributes during training will provide insight into the training process.  


In this paper, we explore how attributes are encoded in the internal layers of both a Resnet-101 and an Inception Resnet v2 architecture based DCNN; and how attribute encoding evolves during training for both these two networks \cite{ranjan2019fast},\cite{bansal2018deep}. To gain a greater understanding of the relationship between attributes, we introduce the concept of \textit{expressivity} of an attribute. Expressivity is a measure of how much a given set of features tells us about an attribute.  If the expressivity between a given set of features and gender is high, then the features can reliably predict gender; if the expressivity for yaw (pose) is low, then yaw cannot be reliably predicted. We define this concept more precisely in Section \ref{sec:expressivity}. 
Below we list the conceptual and experimental contributions of our paper.%\\ 
\begin{enumerate}%[leftmargin=0.1cm]
    \item We are the first to investigate the encoding of facial attributes in the internal layers of DCNNs. 
    \item In the final fully connected layer of both networks, we observed that the order of  expressivity of three facial attributes to be Age $>$ Gender $>$ Yaw.
    \item The expressivity of identity jumps from the last pooling layer to the final fully connected layer. 
    \item For DCNNs, we are the first to monitor the evolution of the encoding of facial attributes during training.
    \item We found that as training progresses, the expressivity of yaw, gender and age decreases, and identity increases. The observed rate of decrease was Age $<$ Gender $<$ Yaw.
    \item We obtained similar results for both Resnet-101 and Inception Resnet v2 architectures.
\end{enumerate}

%\pjp{Prithvi, tomorrow I will write a new concluding paragraph for the introduction.}





==> intro_v3.tex <==
\newcommand{\tcr}[1]{\textcolor{red}{#1}}
\newcommand{\pjp}[1]{\textcolor{red}{#1}}
\newcommand{\prithvi}[1]{\textcolor{blue}{#1}}

\section{Introduction}
\label{sec:intro}

A face image contains information on the identity, gender, age, race of the person, the pose and lighting of the face, and maybe the details of the location where the photo was taken. Deep convolutional neural networks (DCNN)-based face algorithms generate a representation that encodes the identity of the face.  Along with identity, the representation encodes additional information including gender, pose, age, and illumination direction \cite{hill2018deep,DBLP:journals/corr/abs-1904-01219,parde2017face}.  How much information about  facial attributes are captured in the internal layers of the network?  How does the encoding of facial attributes evolve as training progresses?  We address  these two questions.


In this paper, we explore how attributes are encoded in the internal layers of two different and successful architectures: a Resnet-101 and an Inception Resnet v2 architecture based DCNN \cite{ranjan2019fast},\cite{bansal2018deep}.  In addition, we examine how encoding of attributes evolves over training iterations for both these two networks.  To gain a greater understanding of the relationship between attributes, we introduce the concept of \textit{expressivity} of an attribute. Expressivity is a measure of how much a given representation tells us about an attribute, where  the representation of a face can be from internal or final layers in a DCNN.  If the expressivity for gender is high, then gender can be reliably predicted; if the expressivity for yaw (pose) is low, then yaw (pose) cannot be reliably predicted. We define this concept more precisely in Section \ref{sec:expressivity}. 
Below we list the conceptual and experimental contributions of our paper.%\\ 
\begin{enumerate}%[leftmargin=0.1cm]
    \item We are the first to investigate the encoding of facial attributes in the internal layers of DCNNs.
        \item For DCNNs, we are the first to monitor the evolution of the encoding of facial attributes during training.
    \item In the final fully connected layer of both networks, we observed that the order of  expressivity for three facial attributes to be Age $>$ Sex $>$ Yaw.
        \item We found that as training progresses, the expressivity of yaw, gender and age decreases. The observed rate of decrease was Age $<$ Sex $<$ Yaw.
    \item The expressivity of identity dramatically increases from the last pooling layer to the final fully connected layer. 
    \item We obtained similar results for both Resnet-101 and Inception Resnet v2 architectures.
\end{enumerate}

Knowing how face attributes are expressed in both internal layers and during training has both scientific and societal importance. 
Since DCNN-based face recognition systems are fielded in the real-world, the need for these networks to be explainable is pressing.  Understanding how internal layers encode attributes could serves as a basis for explaining identification decisions.
 The ability to  discern important attributes from the final layer is not the final word; it may be possible to discern them from the interior of a network.  For example, our results suggest that the encoding for gender can be stronger in internal layers than the final layer.  From a scientific perspective, knowing the importance of attributes during training will provide insight into the training process.  






